Analysis of a class of Multi-Level Markov Chain Monte Carlo algorithms based on Independent Metropolis-Hastings

In this work, we present, analyze, and implement a class of Multi-Level Markov chain Monte Carlo (ML-MCMC) algorithms based on independent Metropolis-Hastings proposals for Bayesian inverse problems. In this context, the likelihood function involves solving a complex differential model, which is then approximated on a sequence of increasingly accurate discretizations. The key point of this algorithm is to construct highly coupled Markov chains together with the standard Multi-level Monte Carlo argument to obtain a better cost-tolerance complexity than a single-level MCMC algorithm. Our method extends the ideas of Dodwell, et al. "A hierarchical multilevel Markov chain Monte Carlo algorithm with applications to uncertainty quantification in subsurface flow," \textit{SIAM/ASA Journal on Uncertainty Quantification 3.1 (2015): 1075-1108,} to a wider range of proposal distributions. We present a thorough convergence analysis of the ML-MCMC method proposed, and show, in particular, that (i) under some mild conditions on the (independent) proposals and the family of posteriors, there exists a unique invariant probability measure for the coupled chains generated by our method, and (ii) that such coupled chains are uniformly ergodic. We also generalize the cost-tolerance theorem of Dodwell et al., to our wider class of ML-MCMC algorithms. Finally, we propose a self-tuning continuation-type ML-MCMC algorithm (C-ML-MCMC). The presented method is tested on an array of academic examples, where some of our theoretical results are numerically verified. These numerical experiments evidence how our extended ML-MCMC method is robust when targeting some \emph{pathological} posteriors, for which some of the previously proposed ML-MCMC algorithms fail.

==> figures/figures/test.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}[scale=0.7]

\begin{groupplot}[group style={group size=2 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
title={Dof =289},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.2,0.4,0.6,0.8,1},
xticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {figures/test-000.png};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={Dof =1089},
x grid style={white!69.0196078431373!black},
xmin=0, xmax=1,
xtick style={color=black},
xtick={0,0.2,0.4,0.6,0.8,1},
xticklabels={0.0,0.2,0.4,0.6,0.8,1.0},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=1,
ytick style={color=black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=1, ymin=0, ymax=1] {figures/test-001.png};
\end{groupplot}

\end{tikzpicture}


==> sections/error_analysis.tex <==
Let $\ell=1,2,\dots,\mathscr{L},$ $f:\Te^2\mapsto \R$ be a $\nul$-integrable function, and $\nu^0$ be a probability measure on $(\Te^2,\mathcal{B}(\Te^2))$ such that $\nu^0\ll \nul$. In addition, denote by $	\mathsf{E}_{\nu^0, \bm{P}_\ell}[f]$ the expectation of $f$ over the Markov chain generated by $\Pisl$, starting from an initial probability measure $\nu^0$, and consider the following ergodic estimator:
 \begin{align}\label{eq:erg}
\hat{f}_{\ell,N_\ell,n_{b,\ell}}:=\frac{1}{N_\ell}\sum_{n=1}^{N_\ell}f(\tebl^{n+n_{b,\ell}}),\quad \tebln\sim \pisl(\tebl^{n-1},\cdot),
\end{align}
where $n_{b,\ell}\in \mathbb{N}$ is the usual \emph{burn-in period}.  The aim of this section is to provide error bounds on the non-asymptotic Mean Square Error of \eqref{eq:erg}, namely 
\begin{align}
\mathrm{MSE}(\hat{f}_{\ell,N_\ell,n_{b,\ell}};\nu^0):=\left(\mathsf{E}_{\nu^0, \bm{P}_\ell}\left[\hat{f}_{\ell,N_\ell,n_{b,\ell}}-\nul(f)\right]\right)^2.
	\end{align} 
In particular,in order to fulfill \ref{Assumption:for_cost_thm3} in Section \ref{sec:cost_analysis}, we aim at obtaining a bound of the form
 \begin{align}\label{eq:mse_bound_can}
\mathrm{MSE}(\hat{f}_{\ell,N_\ell,n_{b,\ell}};\nu^0)\leq C_{\mathrm{mse},\ell}\frac{\V_{\nul}[f]}{N_\ell},
 \end{align}
for some level-dependent, positive constant $C_{\mathrm{mse},\ell}.$  Such a bound is presented in Theorem \ref{thm:namse}, the main result of this Section. Bounds such as \eqref{eq:mse_bound_can} are known to exists for geometrically ergodic and reversible Markov transition kernels \cite{rudolf2011explicit}. However, the chain generated by $\Pisl$ is not $\nul$-reversible, as shown in Proposition \ref{prop:rev}.
 \begin{proposition} \label{prop:rev}The chain generated by $\pisl$, $\ell=1,2,\dots,\mathscr{L},$ is \emph{not} $\nul$-reversible. 
 	\begin{proof}
 		\todo.
 		\end{proof}
 \end{proposition}
 As a consequence, we can not directly apply the non-asymptotic bounds presented in \cite{rudolf2011explicit}.  Instead, inspired by the error analysis of \cite{rudolf2011explicit} and the so-called \emph{pseudo-spectral} approach of \cite{paulin2015concentration}, we construct a bound of the form \eqref{eq:mse_bound_can} for non-reversible chains in Theorem \ref{thm:namse} \cjp{better wording here?}. To the best of the authors' knowledge, this is the first time a bound of the form \eqref{eq:mse_bound_can} has been presented for non-reversible chains. 
 
   We begin with some definitions. \cjp{In the interest of briefty, i am giving the definitions ``inline'' by \emph{emphasizing} the word being defined, as opposed to the more formal Definition macro...I can change it if you consider  we should} For any $\ell=1,2,\dots,\mathscr{L}$, we define the \emph{$\epsilon$-mixing time} associated to $\Pisl$ as 
 \begin{align}
 	\tau_\ell(\epsilon):=\min_{t\geq1} \left\{ \lno\nu ^0\Pisl^t-\nul\rno_\mathrm{tv}\leq\epsilon\right\},
 \end{align}
 where $\lno \cdot \rno_\mathrm{tv}$ is the usual total variation  norm for probability measures, and $t\in\mathbb{N}$. A consequence of Theorem \ref{thm:main_existence_ergo} is that $\lno \nu^0\bm P_\ell^t-\nu_\ell\rno_\mathrm{tv}\to 0$ as $t\to\infty$.  We will use the convention that $\tau_\ell(1/4)=:\tau_\ell.$
 It is known \cite[Section 3.3]{roberts2004general}  that $\tau_\ell(\epsilon)$ is finite if and only if $\Pisl$ generates a uniformly ergodic chain \cjp{maybe write as a Lemma?}.  Thus, the $\epsilon$-mixing time of the chain generated by $\Pisl$ is finite provided that Assumption {\ref{Ass:positivity}} holds. 
 Moreover, we define the so-called \emph{pseudo-spectral gap} of an operator $\bm G: L_2(\Te^2,\nul)\mapsto  L_2(\Te^2,\nul)$ as
 \begin{align}\label{eq:psg}
 	\gamma_\mathrm{ps}[\bm G]:=\underset{k\geq 1}{\max}\left \{ \gamma_2[ (\bm G^*)^k\bm G^k ]/k \right\},\ k \in \mathbb{N}.
 \end{align}
 
 As mentioned in \cite{paulin2015concentration}, the pseudo-spectral gap can be understood as a generalization of the $L_2$-spectral gap of the  so-called \emph{multiplicative reversibilization} $\bm R_\ell:=(\Psml\Pisl).$     Furthermore, define the \emph{averaging} operator as $\nulop f:=\nul(f)=\int_{\Te^2}f(\tebl)\nul(\diff\tebl).$  
 %Following the setting of \cite{paulin2015concentration}, we define the so-called \emph{time-reversal} of the Markov kernel $\pisl$ as \begin{align}
 %\psml(\tebl,\diff \bm z_\ell):=\frac{\nul(\diff \bm z_\ell)}{\nul(\diff  \tebl)}\pisl(\zel,\diff\tebl),\ \tebl,\zel\in\Te^2,\ell=1,2,\dots,\mathscr{L}.
 %\end{align}
 Lastly, for any $q,q'\in[1,\infty]$ with  $\frac{1}{q}+\frac{1}{q'}=1,$ we denote the \emph{adjoint operator} of $\Pisl:L_q(\Te^2,\nul)\mapsto L_q(\Te^2,\nul)$ by $\Psml:L_{q'}(\Te^2,\nul)\mapsto L_{q'}(\Te^2,\nul).$ It can be shown \cite{rudolf2011explicit} that a Markov operator acting on $L_2(\Te^2,\nul)$ is self-adjoint if and only if it is $\nul$-reversible. Notice that, even though $\Pisl$ is not reversible, the multiplicative reversibilization $\bm R_\ell=(\Psml\Pisl)$ is. 
 \begin{assumption}\label{Ass:l_inf}
 	For any $\ell=1,2,\dots,\mathscr{L},$ the Markov chain generated by $\Pisl$ is started from a measure $\nu^0$ concentrated around the diagonal $\mathcal{D}$. This in turn implies that $\nu^0\ll\nul$, and  $\frac{\diff \nu^0}{\diff \nul}\in L_\infty(\Te^2,\nul).$ 
 \end{assumption}

 The main result of this section is given by Theorem \ref{thm:namse}. 
 \begin{theorem}[Non-asymptotic bound on the mean square error]\label{thm:namse}
 	Suppose Assumptions  \emph{\ref{Ass:positivity}} and \emph{\ref{Ass:l_inf}} hold. In addition, for any level $\ell=1,2,\dots,\mathscr{L}$, let $f\in  L_2(\Te^2,\nul)$, and write $g(\tebl)=f(\tebl)-\int_{\Te^2}f(\tebl)\nul(\diff \tebl)$.  Then,
 	\begin{align}
 	\mathrm{MSE}(\hat{f}_{\ell,N_\ell,n_{b,\ell}};\nu^0)=\mathsf{E}_{\nu^0, \bm{P}_\ell}\left|\frac{1}{N_\ell}\sum_{n=1}^{N_\ell}g(\tebl^{n+n_{b,\ell}})\right|^2\leq\frac{\V_{\nul}[f]}{N_\ell}(C_{\mathrm{inv},\ell}+ C_{\mathrm{ns},\ell}),\label{eq:bound_namse}
 	\end{align}	
 	where $C_{\mathrm{inv},\ell}=\left(1+\frac{4}{\gamma_\mathrm{ps}[\Pisl]}\right),$ $C_{\mathrm{ns},\ell}=\left(2\lno\frac{\diff \nu^0}{\diff \nul}-1 \rno_{L_\infty}\left(1+\frac{4}{\gamma_{\mathrm{ps}}[\Pisl]}\right)\right)$, and $\gamma_{\mathrm{ps}}[\bm P_\ell]$ is the pseudo-spectral gap of $\Pisl,$ defined in \eqref{eq:psg}. 
 \end{theorem}
The bound \eqref{eq:bound_namse} should be compared to the one presented in \cite[Theorem 3.34]{rudolf2011explicit}. In particular, that work presents a sharper bound than \eqref{eq:bound_namse},  however, such a bound necessitates the additional assumptions of (i) the existence of a positive $L_2$-spectral gap and (ii) reversibility of the chain, the latter of which is not satisfied by the chain generated by $\Pisl$.   We will postpone the proof of Theorem \ref{thm:namse} to the end of the next subsection and present first some intermediate results. 
\subsection{proof of Theorem \ref{thm:namse}}
For the bound \eqref{eq:bound_namse} to be meaningful, we clearly need $\gamma_{\mathrm{ps}}[\bm P_\ell]>0$. To that end, we present the following result, which is adapted from \cite{paulin2015concentration}.
\begin{lemma}\label{bound:gam} Suppose Assumption \emph{\ref{Ass:positivity}} holds. Then, \begin{align}
	\gamma_\mathrm{ps}[\bm P_\ell]\geq \frac{1}{2\tau_\ell}>0,
	\end{align}
	where $\tau_\ell\geq1$ is the mixing time of the chain generated by $\Pisl$. 
\begin{proof}
This is \cite[Proposition 3.4]{paulin2015concentration}, which was originally stated for uniformly ergodic chains. Recall that $\Pisl$ generates a uniformly convergent chain provided Assumption \ref{Ass:positivity} holds.
\end{proof}
\end{lemma}


\begin{proposition}
Let $\alpha\in (0,1)$, $k\geq1$, $N\in \mathbb{N}$. Then,
 \begin{align}\alpha^{1/k}&\leq k \alpha \label{eq:bound_alpha1},\\
\sum_{j=1}^{N-1}\sum_{i=j+1}^{N}\alpha^{i-j}&=\frac{(N-1)\alpha-N\alpha^2+\alpha^{N+1}}{(1-\alpha)^2} . \label{eq:bound_alpha_2}\end{align}
\end{proposition}
We now present a first bound of the form \eqref{eq:mse_bound_can} for chains which are started at stationarity, i.e., whenever $\nu^0=\nul$. Although this is usually not the case, the following Lemma will be useful in the proof of Theorem \ref{thm:namse}. 
\begin{lemma}[MSE bound starting at stationarity]\label{lemma:mse_stationarity}
Suppose Assumption \emph{\ref{Ass:positivity}} holds, let $f\in  L_2(\Te^2,\nul)$, write $g(\tebl)=f(\tebl)-\int_{\Te^2}f(\tebl)\nul(\diff \tebl),$ and suppose the Markov chain generated by $\Pisl$ starts from stationarity (i.e., $\tebl^0 \sim \nul$). Then, 

\begin{align}
	\mathrm{MSE}(\hat{f}_{\ell,N_\ell,n_{b,\ell}=0};\nul)=\mathsf{E}_{\nul, \bm{P}_\ell}\left|\frac{1}{N_\ell}\sum_{n=1}^{N_\ell}g(\tebl^{n+n_{b,\ell}})\right|^2\leq \frac{\V_{\nul}[f]}{N_\ell}\left(1+\frac{4}{\gamma_\mathrm{ps}[\Pisl]}\right).
\end{align}



\begin{proof} We follow a similar approach to those presented in \cite[Theorem 3.2]{paulin2015concentration}. In order to ease notation, for the remainder of this proof we write $ L_q= L_q(\Te^2,\nul), \ q\in[1,\infty]$. We can write the MSE of a Markov chain generated by $\Pisl$ starting at $\nul$ as 
\begin{align}
\mathsf{E}_{\nu_\ell, \bm{P}_\ell}\left|\frac{1}{N_\ell}\sum_{n=1}^{N_\ell}g(\tebl^n)\right|^2=\frac{1}{N_\ell^2}\sum_{n=1}^{N_\ell}\mathsf{E}_{\nu_\ell, \bm{P}_\ell}[g(\tebl^n)^2]+\frac{2}{N_\ell^2}\sum_{j=1}^{N_\ell-1}\sum_{i=j+1}^{N_\ell}\mathsf{E}_{\nu_\ell, \bm{P}_\ell}[g(\tebl^i)g(\tebl^j)]. \label{eq:mse_g}
\end{align}
Working on the expectation of the second term on the right hand side we get from the Cauchy-Schwarz inequality  that
\begin{align}
\mathsf{E}_{\nu_\ell, \bm{P}_\ell}[g(\tebl^i)g(\tebl^j)]&=\langle g,\bm{P}^{i-j}_{ \ell}g\rangle_{\nul}=\langle g,(\bm{P}_{ \ell}-\nulop)^{i-j}g\rangle_{\nul}\\
&\leq \lno g\rno_{ L_2}^2 \lno (\bm{P}_{ \ell}-\nulop)^{i-j}\rno_{ L_2\mapsto  L_2}.
\end{align}	
Notice that for any $k\geq 1$,  we have 
\begin{align}
\lno (\bm{P}_{ \ell}-\nulop)^{i-j}\rno_{ L_2\mapsto  L_2}&\leq\lno (\bm{P}_{ \ell}-\nulop)^k\rno_{ L_2\mapsto  L_2}^{\lfloor\frac{i-j}{k}\rfloor}\\
&=\lno(\bm{P}^*_{ \ell}-\nulop)^k (\bm{P}_{ \ell}-\nulop)^k\rno_{ L_2\mapsto  L_2}^{\frac{1}{2}\lfloor\frac{i-j}{k}\rfloor} \label{eq:bound_P}
\end{align}
where $\lfloor\cdot\rfloor$ is the floor function. Now, let $k_\mathrm{ps}$ be the smallest integer such that 
\begin{align}\label{eq:k_ps}
k_\mathrm{ps}\gamma_\mathrm{ps}[\Pisl]=\gamma[(\bm P^*_\ell)^{k_\mathrm{ps}} \bm P^{k_\mathrm{ps}}_\ell]=1-\lno(\bm{P}^*_{ \ell}-\nulop)^{k_\mathrm{ps}} (\bm{P}_{ \ell}-\nulop)^{k_\mathrm{ps}}\rno_{ L_2\mapsto  L_2},
\end{align}
which, is strictly positive by Lemma \ref{bound:gam}.  Then, from \eqref{eq:mse_g}, \eqref{eq:bound_P}, and \eqref{eq:k_ps}, we obtain: 
\begin{align}
&\frac{2}{N_\ell^2}\sum_{j=1}^{N_\ell-1}\sum_{i=j+1}^{N_\ell}\mathsf{E}_{\nu_\ell, \bm{P}_\ell}[g(\tebl^i)g(\tebl^j)]\leq \frac{ 2 }{N_\ell^2}\sum_{j=1}^{N_\ell-1}\sum_{i=j+1}^{N_\ell}\lno g\rno_{ L_2}^2 \left(1-k_\mathrm{ps}\gamma_\mathrm{ps}[\Pisl]\right)^{\frac{1}{2}\lfloor\frac{i-j}{k_\mathrm{ps}}\rfloor}.
\end{align}
Moreover, from \eqref{eq:bound_alpha1} we have $\left(1-k_\mathrm{ps}\gamma_\mathrm{ps}[\Pisl]\right)^{\frac{1}{2}\lfloor\frac{i-j}{k_\mathrm{ps}}\rfloor}\leq 2k_\mathrm{ps}\left(1-k_\mathrm{ps}\gamma_\mathrm{ps}[\Pisl]\right)^{i-j}$. Thus,
\begin{align}
&\frac{ 2 }{N_\ell^2}\sum_{j=1}^{N_\ell-1}\sum_{i=j+1}^{N_\ell}\lno g\rno_{ L_2}^2 \left(1-k_\mathrm{ps}\gamma_\mathrm{ps}[\Pisl]\right)^{\frac{1}{2}\lfloor\frac{i-j}{k_\mathrm{ps}}\rfloor}\leq  
\frac{ 4k_\mathrm{ps}\lno g\rno_{ L_2}^2 }{N_\ell^2}\sum_{j=1}^{N_\ell-1}\sum_{i=j+1}^{N_\ell} \left(1-k_\mathrm{ps}\gamma_\mathrm{ps}[\Pisl]\right)^{i-j}.
\end{align}
Furthermore, applying \eqref{eq:bound_alpha_2} with $\alpha_{\gamma,\ell}=\left(1-k_\mathrm{ps}\gamma_\mathrm{ps}[\Pisl]\right)$ and $N=N_\ell$ we obtain 
\begin{align}
	\frac{ 4k_\mathrm{ps}\lno g\rno_{ L_2}^2 }{N_\ell^2}\sum_{j=1}^{N_\ell-1}\sum_{i=j+1}^{N_\ell} \left(1-k_\mathrm{ps}\gamma_\mathrm{ps}[\Pisl]\right)^{i-j}&=	\frac{ 4k_\mathrm{ps}\lno g\rno_{ L_2}^2 }{N_\ell^2} \frac{(N_\ell-1)\alpha_{\gamma,\ell}-N_\ell\alpha_{\gamma,\ell}^2+\alpha_{\gamma,\ell}^{N_\ell+1}}{(1-\alpha_{\gamma,\ell})^2} \\
&\leq 	\frac{ 4 \lno g\rno_{ L_2}^2 }{N_\ell \gamma_\mathrm{ps}[\bm P_\ell]}. \label{eq:bound_1}
\end{align}
We now shift our attention to the first term in \eqref{eq:mse_g}. Using H\"older's inequality with $q=\infty,\ q'=1$, together with the fact that $\Pisl$ is a weak contraction in $L_q(\Te^2,\nul)$, for any $q\in[1,\infty]$, we obtain 
\begin{align}
\frac{1}{N_\ell^2}\sum_{n=1}^{N_\ell}\mathsf{E}_{\nu_\ell, \bm{P}_\ell}[g(\tebl^n)^2]=\frac{1}{N_\ell^2}\sum_{n=1}^{N_\ell}\langle 1, \bm P ^n_\ell g^2\rangle_{\nul}\leq\frac{1}{N_\ell^2}\sum_{n=1}^{N_\ell}\lno \bm P ^n_\ell g^2 \rno_{L_1}\leq \frac{ \lno g^2\rno_{ L_1}}{N_\ell}.
\end{align}
Lastly, notice that $$\lno g^2\rno_{ L_1}=\int_{\Te^2}|g^2(\tebl)|\nul(\diff \tebl)=\int_{\Te^2}g^2(\tebl)\nul(\diff \tebl)=\lno g\rno^2_{L_2}.$$ Hence, we obtain the bound \begin{align}
\frac{1}{N_\ell^2}\sum_{n=1}^{N_\ell}\mathsf{E}_{\nu_\ell, \bm{P}_\ell}[g(\tebl^n)^2]\leq \frac{ \lno g\rno_{ L_2}^2}{N_\ell}. \label{eq:bound2}
\end{align}  Thus, from \eqref{eq:mse_g}, \eqref{eq:bound_1}, \eqref{eq:bound2}, together with the observation that $\lno g\rno_{L_2}^2=\int_{\Te^2}(f(\tebl)-\nulop(f))^2\nul(\diff \tebl)=\V_{\nul}[f]$, we finally obtain,
\begin{align}
\mathsf{E}_{\nu_\ell, \bm{P}_\ell}\left|\frac{1}{N_\ell}\sum_{n=1}^{N_\ell}g(\tebl^n)\right|^2&\leq \frac{\lno g\rno_{ L_2}^2}{N_\ell} \left(1+\frac{4}{\gamma_\mathrm{ps}[\Pisl]}\right)\\
&=\frac{\V_{\nul}[f]}{N_\ell}\left(1+\frac{4}{\gamma_\mathrm{ps}[\Pisl]}\right).
\end{align}
\end{proof}
\end{lemma}
The previous result should be compared to \cite[Theorem 3.2]{paulin2015concentration} and \cite[Theorem 5]{rudolf2009explicit}. We now consider the more general case where the chain is not started from stationarity, i.e., when $\tebl^0\sim\nu^0$, where $\nu^0\ll\nul$ is a probability measure on $(\Te^2,\mathcal{B}(\Te^2))$. We recall the following result from \cite{rudolf2011explicit}. 
\begin{lemma}\label{lemma:aux_mse}
Suppose Assumption \emph{\ref{Ass:positivity}}  holds. In addition, for any level $\ell=1,2,\dots,\mathscr{L}$, let $f\in  L_2(\Te^2,\nul)$, $g:=f-\nulop(f),$ denote by $n_{b,\ell}\in\mathbb{N}$ the burn-in period of the samples at level $\ell$, and let $\{ \tebln\}_{n\in\mathbb{N}}$ be a Markov chain generated by $\Pisl$ starting from an initial measure $\nu^0$ and invariant probability measure $ \nul$. Then,
\begin{align}
\mathsf{E}_{\nu^0, \bm{P}_\ell}\left|\frac{1}{N_\ell}\sum_{n=1}^{N_\ell}g(\tebl^{n+n_{b,\ell}})\right|^2&=\mathsf{E}_{\nu_\ell, \bm{P}_\ell}\left|\frac{1}{N_\ell}\sum_{n=1}^{N_\ell}g(\tebl^n)\right|^2+\frac{1}{N_\ell^2}\sum_{j=1}^{N_\ell}\mathcal{H}_\ell^{j+\nbl}(g^2)\\&+\frac{2}{N_\ell^2}\sum_{j=1}^{N_\ell-1}\sum_{k=j+1}^{N_\ell}\mathcal{H}_\ell^{j+\nbl}(g\bm{P}^{k-j}_\ell g), \label{eq:mse_ns}
\end{align} 
where \begin{align}
\mathcal{H}^{i}_\ell(h)=\left \langle (\bm P_\ell^i-\nulop)h,\left(\frac{\diff \nu^0}{\diff \nul}-1\right)\right \rangle_{\nul}, \quad i\in \mathbb{N}, \ h\in L_2(\Te^2,\nul), \ \ell=1,2,\dots,\mathscr{L}. \label{eq:hcal}
\end{align}
	\begin{proof}
		See \cite[Proposition 3.29]{rudolf2011explicit}.
		\end{proof}
\end{lemma}
We can now prove Theorem \ref{thm:namse}. 
\begin{proof}[proof of Theorem \ref{thm:namse}] Once again, for the remainder of this proof we write $ L_q= L_q(\Te^2,\nul), \ q\in[1,\infty].$ From Lemma \ref{lemma:aux_mse}  we get 
\begin{align}
\mathcal{H}_\ell^{j+\nbl}(g^2) &=\left \langle (\bm P_\ell^{j+\nbl}-\nulop)g^2,\left(\frac{\diff \nu^0}{\diff \nul}-1\right)\right \rangle_{\nul}, \label{eq:hg2}\\
%
\mathcal{H}_\ell^{j+\nbl}(g\bm{P}^{k-j}_\ell g)&=\left \langle (\bm P_\ell^{j+\nbl}-\nulop)(g\bm{P}^{k-j}_\ell g),\left(\frac{\diff \nu^0}{\diff \nul}-1\right)\right \rangle_{\nul}.\label{eq:hgpg}
\end{align} 	
 Using H\"older's inequality with $q'=\infty$, $q=1$ on the right hand side of \eqref{eq:hg2} gives
 \begin{align}
 \mathcal{H}_\ell^{j+\nbl}(g^2) &\leq  \lno\frac{\diff \nu^0}{\diff \nul}-1 \rno_{L_\infty} \lno (\bm P_\ell^{j+\nbl}-\nulop)g^2 \rno_{L_1} \\
 &\leq  \lno\frac{\diff \nu^0}{\diff \nul}-1 \rno_{L_\infty} \lno (\bm P_\ell^{j+\nbl}-\nulop)\rno_{L_1\mapsto L_1}\lno g^2 \rno_{L_1} \label{eq:hg22},
 \end{align} 
 where the last inequality comes from the definition of operator norm. Moreover, since the Markov operators are weak contractions, we have that $\lno (\bm P_\ell^{j+\nbl}-\nulop)\rno_{L_1\mapsto L_1}\leq 2, \forall j\in\mathbb{N}$. Furthermore, it can be seen that \begin{align}
 \lno g^2\rno_{L_1}=\int_{\Te^2}|g^2(\tebl)|\nul(\diff \tebl)=\int_{\Te^2}g(\tebl)^2\nul(\diff \tebl)=\lno g\rno_{L_2}^2,
 \end{align}
 which gives the bound 
 \begin{align}
 \mathcal{H}_\ell^{j+\nbl}(g^2)\leq  2\lno\frac{\diff \nu^0}{\diff \nul}-1 \rno_{L_\infty} \lno g \rno_{L_2}^2.
 \end{align}
 Summing over $j$ gives 
\begin{align}
\frac{1}{N_\ell^2}\sum_{j=1}^{N_\ell} \mathcal{H}_\ell^{j+\nbl}(g^2) \leq \frac{2\lno g \rno_{L_2}^2}{N_\ell}\lno\frac{\diff \nu^0}{\diff \nul}-1 \rno_{L_\infty}. \label{eq:hg23}
\end{align}
Following similar procedure for \eqref{eq:hgpg} we obtain
\begin{align}
 \mathcal{H}_\ell^{j+\nbl}(g\bm P_\ell^{k-j}g)\leq 2 \lno\frac{\diff \nu^0}{\diff \nul}-1 \rno_{L_\infty} \lno g(\bm P_\ell^{k-j})g \rno_{L_1}. \label{eq:Hgpg2}
\end{align}
Furthermore, from H\"older's inequality (with $q'=q=2)$ and the fact that $\nulop(g)=0$ we get
 \begin{align}
\lno g(\bm P_\ell^{k-j})g \rno_{L_1}&\leq \lno g \rno_{L_2}\lno \bm P_\ell^{k-j}g\rno_{L_2} 
= \lno g \rno_{L_2}\lno (\bm P_\ell-\nulop)^{k-j}g\rno_{L_2}\\&\leq \lno g \rno_{L_2}^2\lno (\bm P_\ell-\nulop)^{k-j}\rno_{L_2\mapsto L_2}\leq\lno g \rno_{L_2}^2\left(1-k_\mathrm{ps}\gamma_\mathrm{ps}[\Pisl]\right)^{k-j},
\end{align}
where the last inequality follows from the same pseudo-spectral gap argument used in the proof of Lemma \ref{lemma:mse_stationarity}. Adding over $j$ and $k$ gives 
\begin{align}
\frac{2}{N_\ell^2}\sum_{j=1}^{N_\ell-1}\sum_{k=j+1}^{N_\ell}\mathcal{H}_\ell^{j+\nbl}(g\bm{P}^{k-j}_\ell g)\leq \frac{8\lno g\rno_{L_2}^2}{N_\ell \gamma_{\mathrm{ps}}}\lno\frac{\diff \nu^0}{\diff \nul}-1 \rno_{L_\infty} \label{eq:Hgpg3}.
\end{align}
Notice then that Equations \eqref{eq:hg23} and \eqref{eq:Hgpg3}, provide a bound on the second and third term in Lemma \ref{lemma:aux_mse}. Lastly, combining these results with Lemma \ref{lemma:mse_stationarity} and once again observing that $\lno g\rno_{L_2}^2=\V_{\nul}[f]$, gives  the desired result
\begin{align}
&\eqref{eq:mse_ns}\leq \frac{\V_{\nul}[f]}{N_\ell}\left(1+\frac{2}{\gamma_\mathrm{ps}[\Pisl]}\right) +\frac{\V_{\nul}[f]}{N_\ell}\left(2\lno\frac{\diff \nu^0}{\diff \nul}-1 \rno_{L_\infty}\left(1+\frac{4}{\gamma_{\mathrm{ps}}[\bm P_\ell]}\right)\right).
\end{align}
		\end{proof}
	
	

% We follow an approach similar the so-called \emph{first Metropolis kernel} presented in \cite{choi2020metropolis}. We begin by defining an auxiliary function.
%\begin{definition}[Nested acceptance rate]	For any given level $\ell=1,2,\dots,\mathscr{L}$, we define the  \emph{nested acceptance ratio} at level $\ell,$  $\anl:\Te^2\times \Te^2\mapsto[0,1]$ as 
%	\begin{align}
%	\anl(\tebl,\zb):=\min\left\{ 1, \frac{\nul(\zb)\pisl(\zb,\tebl)}{\nul(\tebl)\pisl(\tebl,\zb)}  \right\}, \label{eq:alpha_nes}
%	\quad \tebl,\zb\in \Te^2.
%	\end{align}
%\end{definition}
%Notice that \eqref{eq:alpha_nes} is the acceptance probability of a Metropolis-Hastings algorithm which uses a proposal $\pisl$ to sample from a probability measure $\nul.$ This is the idea behind the \emph{first Metropolis-Hastings kernel} presented in \cite{choi2020metropolis}; to examine an auxiliary chain which uses $\pisl$ as a proposal. 
%\begin{definition}[Nested kernel] For any given level $\ell=1,2,\dots,\mathscr{L}$, we define the  \emph{nested Markov transition kernel} at level $\ell,$  $\knl:\Te^2\times \calb(\Te^2)\mapsto[0,1]$ as 
%	\begin{align}
%	\knl(\tebl,\dzb):=\anl(\tebl,\zb)\pisl(\tebl,\dzb)+\delta_{\tebl}(\dzb)\left(\int_{\Te^2}1-\anl(\tebl,\bm u)\right)\pisl(\tebl,\diff \bm u), \quad \tebl\in\Te^2.\label{eq:nested_kernel}
%	\end{align}
%	Furthermore, we will denote by $\Knl$ the Markov transition operator associated to $\knl.$
%\end{definition}
%\begin{remark}
%This construction is referred to as \emph{the first Metropolis-Hastings kernel} in \cite{choi2020metropolis}, where, in their context, a so-called \emph{second Markov Metropolis kernel} exists. Given that we will not make use of this second MH kernel, we will refer to the first kernel as the \emph{nested} MH kernel. 
%\end{remark}	
%
%\cjp{this will be moved to the preliminaries. We also need to define $ L_2(\Te^2,\nul)$.}
%
%%\begin{definition}[Peskun ordering]Let $P_1,P_2$ be two $\nul-$invariant Markov operators with $P_j: L_2(\Te^2,
%%	\nul)\mapsto  L_2(\Te_2,\nul), j=1,2$. We say that $P_1$ 
%%	\emph{dominates $P_2$ off the diagonal}, denoted by $P_1\succeq P_2,$ If $\forall A\in\calb(\Te^2)$ \begin{align}
%%	p_1(\tebl,A)\geq p_2(\tebl,A), \quad \tebl\notin A,
%%	\end{align}
%%	where we have denoted by $p_j$ the Markov transition kernel associated to $P_j$, $j=1,2$.
%%\end{definition}	
%
%We now present two theoretical properties of $\knl$. 
%
%\begin{lemma}
%Let $\Knl$ be the Markov operator of the nested kernel \eqref{eq:nested_kernel}. For any given $\ell=1,2,\dots,\mathscr{L},$ the following properties hold:\begin{enumerate}
%	\item $\Knl$ is a $\nul$-reversible Markov operator.
%	\item  $\langle \Pisl f,f\rangle_{\nul}\leq\langle \Knl f,f\rangle_{\nul} \quad \forall f\in  L_2(\Te^2,\nul),$
%\end{enumerate}
%where for any two $\nul$ measurable functions $f,g:\Te^2\mapsto\R$, $\langle f,g\rangle_{\nul}:=\int_{\Te^2}f(\tebl)g(\tebl)\nul(\diff \tebl)$.
%\begin{proof}
%	See \cite[Lemma 3.2]{choi2020metropolis}.
%\end{proof}
%\end{lemma}
%
%
%
%\cjp{So what we want to do is to find a lower bound on $\phi$ such that $\lno \Knl \rno$ has a spectral gap and we can use the theory of Rudolf Lemma 3.26 to 3.32}. 
%
%\begin{lemma}\emph{(Bound on $\Knl$)}
%	
%\end{lemma}		
%	
%\begin{lemma}\emph{(Non-asymptotic bound on mean-square error)}
%	
%\end{lemma}		
%	
	



==> sections/reliability_ell.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.203921568627451,0.541176470588235,0.741176470588235}

\begin{axis}[
axis line style={white!73.7254901960784!black},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
log basis x={10},
log basis y={10},
minor xtick={8e-05,0.00012,0.00014,0.00016,0.00018,0.0002,0.00022},
minor xticklabels={\(\displaystyle {8\times10^{-5}}\),\(\displaystyle {1.2\times10^{-4}}\),\(\displaystyle {1.4\times10^{-4}}\),\(\displaystyle {1.6\times10^{-4}}\),\(\displaystyle {1.8\times10^{-4}}\),\(\displaystyle {2\times10^{-4}}\),\(\displaystyle {2.2\times10^{-4}}\)},
tick pos=left,
x grid style={white!69.8039215686274!black},
xlabel={\(\displaystyle \mathsf{tol}\)},
xmajorgrids,
xmin=9.65936328924845e-05, xmax=0.000207052984768275,
xminorgrids,
xmode=log,
xtick style={color=black},
xtick={1e-06,1e-05,0.0001,0.001,0.01},
xticklabels={\(\displaystyle {10^{-6}}\),\(\displaystyle {10^{-5}}\),\(\displaystyle {10^{-4}}\),\(\displaystyle {10^{-3}}\),\(\displaystyle {10^{-2}}\)},
y grid style={white!69.8039215686274!black},
ylabel={\(\displaystyle \mathsf{te}^2\)},
ymajorgrids,
ymin=9.45417186857789e-10, ymax=4.78089657134172e-08,
yminorgrids,
ymode=log,
ytick style={color=black},
ytick={1e-11,1e-10,1e-09,1e-08,1e-07,1e-06},
yticklabels={\(\displaystyle {10^{-11}}\),\(\displaystyle {10^{-10}}\),\(\displaystyle {10^{-9}}\),\(\displaystyle {10^{-8}}\),\(\displaystyle {10^{-7}}\),\(\displaystyle {10^{-6}}\)}
]
\addplot [very thick, color0]
table {%
0.0002 4e-08
0.00018 3.24e-08
0.00015 2.25e-08
0.0001 1e-08
};
\addlegendentry{$\mathsf{tol}_i^2$}
\addplot [very thick, black, mark=*, mark size=3, mark options={solid}, only marks]
table {%
0.0002 2.01267712238018e-08
0.0002 2.97282243280951e-08
0.0002 2.69872957243336e-08
0.0002 2.60870735890286e-08
0.0002 3.60530690158022e-08
0.0002 2.10378992222268e-08
0.0002 3.29226338214033e-08
0.0002 3.44384950577538e-08
0.0002 1.63190069950531e-08
0.0002 3.93545576144036e-08
0.0002 2.20145988951694e-08
0.0002 1.48636918224377e-08
0.0002 1.1376120495524e-08
0.0002 1.67962402663254e-08
0.0002 5.21167278374428e-09
0.0002 6.140272381678e-09
0.0002 2.14005611776336e-09
0.0002 1.61419487628682e-09
0.0002 1.66079584342907e-08
0.0002 2.7674456063964e-08
};
\addlegendentry{$\mathsf{te}^2$}
\addplot [very thick, red, mark=x, mark size=3, mark options={solid}, only marks]
table {%
0.0002 2.03747144364543e-08
};
\addlegendentry{mean error}
\addplot [very thick, black, mark=*, mark size=3, mark options={solid}, only marks, forget plot]
table {%
0.00018 7.83800794841466e-09
0.00018 1.18049816057172e-08
0.00018 3.03277307888708e-08
0.00018 2.94459344369317e-08
0.00018 2.98538915086659e-08
0.00018 2.95457628577614e-08
0.00018 1.22628465917606e-08
0.00018 1.3440584251678e-08
0.00018 1.02156390336823e-08
0.00018 2.3241044368473e-08
0.00018 2.34802472650898e-08
0.00018 2.68512654056436e-08
0.00018 1.9657411195257e-08
0.00018 7.13898130224648e-09
0.00018 1.43772238561956e-09
0.00018 1.14020530745256e-08
0.00018 2.23154360593231e-08
0.00018 1.36938708110446e-08
0.00018 1.95895828948195e-08
0.00018 1.73525621905173e-08
};
\addplot [very thick, red, mark=x, mark size=3, mark options={solid}, only marks, forget plot]
table {%
0.00018 1.80447777988021e-08
};
\addplot [very thick, black, mark=*, mark size=3, mark options={solid}, only marks, forget plot]
table {%
0.00015 9.11483634389188e-09
0.00015 8.16328267457988e-09
0.00015 1.1798251794177e-08
0.00015 1.41415692803107e-08
0.00015 1.17095845940797e-08
0.00015 1.33093802642203e-08
0.00015 3.97999767633719e-09
0.00015 2.01422871358255e-09
0.00015 1.18134070608555e-08
0.00015 1.12998544678398e-09
0.00015 1.7544506831956e-08
0.00015 1.74137283777098e-09
0.00015 1.68149679553536e-08
0.00015 1.96065208557668e-08
0.00015 4.96754805304961e-09
0.00015 1.36999936966116e-08
0.00015 1.3032383317688e-08
0.00015 1.32954395481553e-08
0.00015 1.32691873271467e-08
0.00015 8.89464545536714e-09
};
\addplot [very thick, red, mark=x, mark size=3, mark options={solid}, only marks, forget plot]
table {%
0.00015 1.05020544863842e-08
};
\addplot [very thick, black, mark=*, mark size=3, mark options={solid}, only marks, forget plot]
table {%
0.0001 4.15850078375701e-09
0.0001 8.06329533340353e-09
0.0001 9.33870496856047e-09
0.0001 6.87898549364076e-09
0.0001 3.90020904489734e-09
0.0001 1.722853356181e-09
0.0001 4.78302108321997e-09
0.0001 4.74265866567246e-09
0.0001 7.83186468263463e-09
0.0001 9.52541654705022e-09
0.0001 4.48980359669929e-09
0.0001 9.2245181516736e-09
0.0001 9.1747196262457e-09
0.0001 6.48657890627853e-09
0.0001 3.77550823265742e-09
0.0001 9.97071699322218e-09
0.0001 1.34516369730555e-09
0.0001 3.78592853045245e-09
0.0001 3.78592853045245e-09
0.0001 3.78592853045245e-09
};
\addplot [very thick, red, mark=x, mark size=3, mark options={solid}, only marks, forget plot]
table {%
0.0001 5.83851523772285e-09
};
\end{axis}

\end{tikzpicture}

